Interfacial polyconvex energy-enhanced evolutionary model for shape memory alloys

A sharp-interface model describing static equilibrium configurations of shape mory alloys by means of interfacial polyconvex energy density introduced by \v{S}ilhav\'y in 2010 and extended to a quasistatic situation by Kn\"upfer and Kru\v{z}\'ik in 2016 is computationally tested. Elastic properties of variants of martensite and the austenite are described by polyconvex energy density functions. Volume fractions of particular variants are modeled by a map of bounded variation. Additionally, energy stored in martensite-martensite and austenite-martensite interfaces is measured by an interface-polyconvex function. It is assumed that transformations between material variants are accompanied by energy dissipation which, in our case, is positively and one-homogeneous giving rise to a rate-independent model. Various two-dimensional computational examples are presented and the used computer code is made available for downloads.

==> article math mech sol/all-def.tex <==
\parindent=0cm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}

\newenvironment{bb}{ \begin{beamerboxesrounded}{} }{ \end{beamerboxesrounded} }
% new itemize environment with itemsep parameter
\newenvironment{myitemize}[1][0]
  { \begin{itemize}
    \addtolength{\itemsep}{#1\baselineskip} % spacing between items
    \addtolength{\baselineskip}{#1\baselineskip} } % spacing between lines
  { \end{itemize} }
\newenvironment{myenumerate}[1][0]
  { \begin{enumerate}
    \addtolength{\itemsep}{#1\baselineskip} % spacing between items
    \addtolength{\baselineskip}{#1\baselineskip} } % spacing between lines
  { \end{enumerate} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Ana 1 Kuerzel
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%COMMAND SHORTCUTS
\newcommand{\qqquad}[0]{\qquad\qquad}
\newcommand{\qqqquad}[0]{\qqquad\qqquad}
\newcommand{\NT}[0]{\notag}
\newcommand{\FA}[1]{\text{für alle $#1$}} 
\newcommand{\FU}[1]{\text{für $#1$}}
\newcommand{\FL}[1]{\text{falls $#1$}}
\newcommand{\ddx}[0]{{\frac d{dx}}}
\newcommand{\ddxk}[1]{{\frac {d^{#1}}{dx^{#1}}}}
\newcommand{\ddtk}[1]{{\frac {d^{#1}}{dt^{#1}}}}
\newcommand{\dde}{{\frac {d}{d\eps}}}
\newcommand{\HW}[1]{} %{\paragraph{Vorschlag für Uebungsaufgabe.}}
\newcommand{\UA}[0]{\"Ubung} %{\paragraph{Vorschlag für \"Ubungsaufgabe.}}


\newcommand{\UI}[1]{ \marginparsep = 1.5mm %Abstand der Randnote zum Text
  \marginpar{\raggedright\footnotesize\itshape \color{blue}{HW: #1} \par} } %
\newcommand{\ER}[1]{ \marginparsep = 1.5mm %Abstand der Randnote zum Text
  \marginpar{\raggedright\footnotesize\itshape \color{green}{[#1]} \par} }
\newcommand{\UAI}[1]{ \UA \UI{#1} } %


\newcommand{\HA}[0]{\"Ubungszettel} %{\paragraph{Vorschlag für \"Ubungsaufgabe.}}
\newcommand{\IDEE}[1]{}
\def\und{\hskip5mm\text{und}\hskip5mm} 
\allowdisplaybreaks[3]
\newcommand{\EMMM}[1]{\underline{#1}} 
\renewcommand{\em}[1]{{\EMMM{#1}}}
\def\ED{\end{document}}



% Equationlist with left brackets
\newenvironment{TC} {\left \{\begin{array}{ll}} {\end{array} \right.}
% Proof with several steps (i),(ii),...
\newcounter{pcounter} 
\newenvironment{penum}{
  \begin{list}{zu (\roman{pcounter}):}{\usecounter{pcounter}}
  }{
  \end{list}
} 
% Proof with several steps Schritt 1,...
\newenvironment{pstep}{
  \begin{list}{\it{Schritt \arabic{pcounter}:}}{\usecounter{pcounter}}
  }{
  \end{list}
}
% Proof of equivalent statements
\newenvironment{pdir}{
  \begin{list}{zu (\roman{pcounter}):}{\usecounter{pcounter}}
  }{
  \end{list}
}%
 \def\LRCITE{``$\Longrightarrow$'':} \def\RLCITE{``$\Longleftarrow$'':}


\newcommand{\RA}[0]{\Rightarrow} \newcommand{\LA}[0]{\Leftarrow}
\newcommand{\LRA}[0]{\Leftrightarrow} \newcommand{\BS}[0]{\backslash}

\newcommand{\toto}[0]{\rightrightarrows}


% Big arrows 
\newcommand{\BRA}[0]{\quad \Longrightarrow \quad} %
\newcommand{\BLRA}[0]{\quad \Longleftrightarrow \quad} % 
\newcommand{\BLA}[0]{\quad \Longleftarrow \quad} %
\newcommand{\OL}[0]{\overline} %
\newcommand{\DBLRA}[0]{\quad :\Longleftrightarrow \quad} % 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% kurz
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\t}{\tilde}
\newcommand{\p}{\partial}
\renewcommand{\d}{\delta}
\newcommand{\e}{\eps}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% mathcal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\AA}{{\mathcal A}}
\newcommand{\BB}{{\mathcal B}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\DD}{{\mathcal D}}
\newcommand{\EE}{{\mathcal E}}
\newcommand{\FF}{{\mathcal F}}
\newcommand{\GG}{{\mathcal G}}
\newcommand{\HH}{{\mathcal H}}
\newcommand{\II}{{\mathcal I}}
\newcommand{\JJ}{{\mathcal J}}
\newcommand{\KK}{{\mathcal K}}
\newcommand{\LL}{{\mathcal L}}
\newcommand{\MM}{{\mathcal M}}
\newcommand{\NN}{{\mathcal N}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\PP}{{\mathcal P}}
\newcommand{\QQ}{{\mathcal Q}}
\newcommand{\RR}{{\mathcal R}}
\renewcommand{\SS}{{\mathcal S}}
\newcommand{\TT}{{\mathcal T}}
\newcommand{\UU}{{\mathcal U}}
\newcommand{\VV}{{\mathcal V}}
\newcommand{\WW}{{\mathcal W}}
\newcommand{\XX}{{\mathcal X}}
\newcommand{\YY}{{\mathcal Y}}
\newcommand{\ZZ}{{\mathcal Z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% mathhbb und mathbf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Q}{\mathbb{Q}}

\newcommand{\qqq}{{\mathbf q}}
\newcommand{\xxx}{{\mathbf x}}
\newcommand{\yyy}{{\mathbf y}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Greek symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\alp}{\alpha}
\newcommand{\bet}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\eps}{\epsilon}
\newcommand{\zet}{\zeta}
\newcommand{\kap}{\kappa}
\newcommand{\lam}{\lambda}
\renewcommand{\phi}{\varphi}
\newcommand{\ome}{\omega}
\newcommand{\sig}{\sigma}

\newcommand{\Gam}{\Gamma}
\newcommand{\Lam}{\Lambda}
\newcommand{\Sig}{\Sigma}
\newcommand{\Ome}{\Omega}

\newcommand{\pOme}{\partial \Omega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Math Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\nin}{\not\in}

\DeclareMathOperator*{\dv}{\ \nabla \- \cdot \-}
\DeclareMathOperator*{\DIV}{div} 
\DeclareMathOperator*{\argmax}{argmax} 
\DeclareMathOperator*{\arcsinh}{arcsinh}
\DeclareMathOperator*{\arccosh}{arccosh}
\DeclareMathOperator*{\cof}{cof} 
\DeclareMathOperator*{\diam}{diam}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\dist}{dist} 
\DeclareMathOperator*{\grad}{grad} 
\DeclareMathOperator*{\Hess}{Hess}
\DeclareMathOperator*{\rot}{rot} 

\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\length}{length}
\DeclareMathOperator*{\osc}{osc} 
\DeclareMathOperator*{\kernel}{kern}
\DeclareMathOperator*{\image}{im}
\DeclareMathOperator*{\graph}{graph}
\DeclareMathOperator*{\id}{id}

\DeclareMathOperator*{\Mat}{Mat} 
\DeclareMathOperator*{\Res}{Res} 
\DeclareMathOperator*{\SO}{SO} 
\DeclareMathOperator*{\Sym}{Sym} 
\DeclareMathOperator*{\Skew}{{Skew}} 
\DeclareMathOperator*{\GL}{{GL}} 
\DeclareMathOperator*{\Id}{{Id}} 
\DeclareMathOperator*{\rang}{{rang}} 


\def \wto{\rightharpoonup}
%\renewcommand{\Re}{\mathfrak{Re}}
%\renewcommand{\Im}{\mathfrak{Im}}
\newcommand{\da}{\partial}
\newcommand{\dd}{\, {\rm d}}
\newcommand{\ddt}{\, \frac{d}{dt}}
\renewcommand{\iint}{\int\!\!\!\!\int}
\newcommand{\gauss}[1]{\lfloor #1 \rfloor}                        % abrunden
\newcommand{\avg}[1]{\langle #1 \rangle}
\newcommand{\avgL}[2]{\langle #1 \rangle_{#2}}
\newcommand{\spann}[1]{{\rm span} \langle \text{$#1$} \rangle}



% Mean value
\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
\vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}

% \upref, \upeq

\newcommand{\upref}[2]{\hspace{-0.8ex}\stackrel{\eqref{#1}}{#2}} % standard
\newcommand{\xupref}[2]{\hspace{-0.3ex}\stackrel{\eqref{#1}}{#2}} % for (x)
\newcommand{\upupref}[3]{\hspace{-3ex}\stackrel{\eqref{#1},\eqref{#2}}{#3}}
\newcommand{\upeq}[2]{\stackrel{#1}{#2}}
\newcommand{\uptext}[2]{\stackrel{\text{#1}}{#2}}

\newcommand{\lupref}[2]{\hspace{0ex} \stackrel{\eqref{#1}}{#2}} % in line
\newcommand{\lupupref}[3]{\hspace{0ex}\stackrel{\eqref{#1},\eqref{#2}}{#3}}
\newcommand{\luptext}[2]{\hspace{0ex} \stackrel{\text{#1}}{#2}} % in line

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEU Farbe
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{color}
% blue
\definecolor{verylightblue}{rgb}{0.95, 0.95, 0.95}  %{0.9 0.95 1}
\definecolor{lightblue}{rgb}{0.7, 0.7, 1}

% yellow
\definecolor{eqyellow}{rgb}{0.9375,0.8984,0.5469}
\definecolor{subeqyellow}{rgb}{1,0.9373,0.8353}

% green
\definecolor{mygreen}{rgb}{0.3, 0.6, 0.3} %{0.9 1 0.9}
\definecolor{verylightgreen}{rgb}{0.95, 0.95, 0.95} %{0.9 1 0.9}
\definecolor{verydarkgreen}{rgb}{0, 0.5, 0}
\definecolor{darkgreen}{rgb}{0.85, 0.85, 0.85}  %{0 0.5 0}
\definecolor{mydarkgreen}{rgb}{0, 0.5, 0} %{0.9 1 0.9}

%brown
\definecolor{mybrown}{rgb}{0.85, 0.4, 0.3}
\definecolor{verylightbrown}{rgb}{0.98, 0.72, 0.58}
\definecolor{verydarkbrown}{rgb}{0.44, 0.26, 0.26}

% orange
\definecolor{orange}{rgb}{1, 0.5, 0}
\newcommand{\orange}[1]{{\color{orange}{#1}}}
\definecolor{BurntOrange}{rgb}{1,0.356,0}
\newcommand{\BurntOrange}{\color{BurntOrange}}

%red
\definecolor{mydarkred}{rgb}{1,0.086,0.255}
\newcommand{\mydarkred}{\color{mydarkred}}
\definecolor{RoseVYDP}{rgb}{0.84,0.086,0.255}
\newcommand{\RoseVYDP}{\color{RoseVYDP}}
\definecolor{dgreen}{rgb}{0, 0.8, 0.5}     
\newcommand{\dgreen}{\color{dgreen}}
\definecolor{CanaryBRT}{rgb}{1,0.76,0.26}
\newcommand{\CanaryBRT}{\color{CanaryBRT}}

% other
\definecolor{cyan}{rgb}{0, 1, 1}
\definecolor{verylightgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{verylightgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{verylightred}{rgb}{1, 0.8, 0.78}
\definecolor{verylightyellow}{rgb}{0.99, 0.98, 0.5}


%\newcommand{\black}{\color{black}}
%\newcommand{\white}{\color{white}}
\newcommand{\mygreen}{\color{mygreen}}
\newcommand{\mydarkgreen}{\color{mydarkgreen}}
\newcommand{\mybrown}{\color{mybrown}}
%\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
%\newcommand{\green}[1]{{\color{green}{#1}}}
\newcommand{\darkgreen}[1]{{\color{darkgreen}{#1}}}
%\newcommand{\cyan}[1]{{\color{cyan}{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% edit
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\edit}[1]{{\color{red}{#1}}}
\newcommand{\short}[1]{{\color{orange}{#1}}}
\newcommand{\ignore}[1]{{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flush right without line break  "\signed"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\parindent0em

\newcommand{\signed}[1]{%
  \unskip\hspace*{1em plus 1fill}%
  \nolinebreak[3]\hspace*{\fill}\mbox{\upshape #1}
}

\newenvironment{xquote}{%
  \begin{list}{}{%
    \rightmargin
    \leftmargin
  }
  \itshape
  \item[]
}
{\end{list}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Standard norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\nco}[1]{\|#1\|_{L^\infty}}
\newcommand{\ncoL}[2]{\|#1\|_{L^\infty({#2})}}
\newcommand{\nck}[2]{\|#1\|_{C^{#2}}}

\newcommand{\nlt}[1]{\|#1\|_{L^2}}
\newcommand{\nltL}[2]{\|#1\|_{L^2({#2})}}

\newcommand{\nbv}[1]{\|#1\|_{BV}}
\newcommand{\nbvL}[2]{\|#1\|_{BV({#2})}}


\newcommand{\cci}{C_c^{\infty}(\R)}
\newcommand{\cciL}[1]{C_c^{\infty}(#1)}

\newcommand{\cii}{C^{\infty}(\R)}
\newcommand{\ciiL}[1]{C^{\infty}(#1)}

\newcommand{\nlo}[1]{\|#1\|_{L^1}}
\newcommand{\nloL}[2]{\|#1\|_{L^1({#2})}}

\newcommand{\NNN}[2]{\|#1\|_{#2}}
\newcommand{\MMM}[2]{[#1]_{#2}}
\newcommand{\skp}[2]{\langle #1, #2 \rangle}
\newcommand{\skpL}[3]{(#1, #2)_{#3}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% H-norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\HS}[1]{H_{#1}}
\newcommand{\HM}[2]{[#1]_{\HS{#2}}}
\newcommand{\HN}[2]{\|#1\|_{\HS{#2}}}
\newcommand{\HP}[3]{\langle #1, #2 \rangle_{\HS{#3}}}

\newcommand{\HSL}[2]{\HS{#1}({#2})}
\newcommand{\HML}[3]{[#1]_{\HSL{#2}{#3}}}
\newcommand{\HNL}[3]{\|#1\|_{\HSL{#2}{#3}}}
\newcommand{\HPL}[4]{\langle #1, #2 \rangle_{\HSL{#3}{#4}}}

\newcommand{\HSS}[1]{\HS_{#1*}}
\newcommand{\HMS}[2]{[#1]_{\HSS{#2}}}
\newcommand{\HNS}[2]{\|#1\|_{\HSS{#2}}}
\newcommand{\HPS}[3]{\langle #1, #2 \rangle_{\HSS{#3}}}

\newcommand{\HSP}[1]{H_{#1}^+}
\newcommand{\HNP}[2]{\|#1\|_{\HSP{#2}}}
\newcommand{\HSM}[1]{H_{#1}^-}
\newcommand{\HNM}[2]{\|#1\|_{\HSM{#2}}}

%\newcommand{\HSo}[1]{H_{0}^{#1}}
%\newcommand{\HMo}[2]{[#1]_{\HS{#2}}}
%\newcommand{\HNo}[2]{\|#1\|_{\HS{#2}}}

\newcommand{\HSoo}[1]{\mathring{H}_{#1}}
\newcommand{\HMoo}[2]{[#1]_{\HS{#2}}}
\newcommand{\HNoo}[2]{\|#1\|_{\HS{#2}}}

\newcommand{\HSooL}[2]{\mathring H_{#1}({#2})}
\newcommand{\HMooL}[3]{[#1]_{\HSooL{#2}{#3}}}
\newcommand{\HNooL}[3]{\|#1\|_{\HSooL{#2}{#3}}}
\newcommand{\HPooL}[4]{\langle #1, #2 \rangle_{\HSooL{#3}{#4}}}

%% time-space

% H^k

\newcommand{\THS}[1]{L^2(\HS{#1})}
\newcommand{\THM}[2]{[#1]_{\THS{#2}}}
\newcommand{\THN}[2]{\|#1\|_{\THS{#2}}}

\newcommand{\THSK}[2]{H^{#1}(\HS{#2})}
\newcommand{\THMK}[3]{[#1]_{\THSK{#2}{#3}}}
\newcommand{\THNK}[3]{\|#1\|_{\THSK{#2}{#3}}}

\newcommand{\THSS}[1]{L^2(\HSS{#1})}
\newcommand{\THMS}[2]{[#1]_{\THSS{#2}}}
\newcommand{\THNS}[2]{\|#1\|_{\THSS{#2}}}

% C^k

\newcommand{\CHS}[1]{C^0(\HS{#1})}
\newcommand{\CHM}[2]{[#1]_{\CHS{#2}}}
\newcommand{\CHN}[2]{\|#1\|_{\CHS{#2}}}

\newcommand{\CHSK}[2]{C^{#1}(\HS{#2})}
\newcommand{\CHMK}[3]{[#1]_{\CHSK{#2}{#3}}}
\newcommand{\CHNK}[3]{\|#1\|_{\CHSK{#2}{#3}}}

\newcommand{\CHSS}[1]{C^0(\HSS{#1})}
\newcommand{\CHMS}[2]{[#1]_{\CHSS{#2}}}
\newcommand{\CHNS}[2]{\|#1\|_{\CHSS{#2}}}

%% parabolic

\newcommand{\PHS}[1]{TH_{#1}}
\newcommand{\PHM}[2]{[#1]_{\dot \PHS{#2}}}
\newcommand{\PHN}[2]{\|#1\|_{\PHS{#2}}}

\newcommand{\PHSL}[2]{TH_{#1}({#2})}
\newcommand{\PHML}[3]{[#1]_{\dot \PHSL{#2}{#3}}}
\newcommand{\PHNL}[3]{\|#1\|_{\PHSL{#2}{#3}}}


%% parabolic-from 0

\newcommand{\PHSN}[1]{\PHS{#1} \cap L^2(H_\eps^0)}
\newcommand{\PHMN}[2]{[#1]_{\dot \PHSN{#2}}}
\newcommand{\PHNN}[2]{\|#1\|_{\PHSN{#2}}}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% X-norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\XS}[1]{X_{#1}}
\newcommand{\XM}[2]{[#1]_{\XS{#2}}}
\newcommand{\XN}[2]{\|#1\|_{\XS{#2}}}
\newcommand{\XP}[3]{\langle #1, #2 \rangle_{\XS{#3}}}

\newcommand{\XSL}[2]{X_{#1}({#2})}
\newcommand{\XML}[3]{[#1]_{\XSL{#2}{#3}}}
\newcommand{\XNL}[3]{\|#1\|_{\XSL{#2}{#3}}}
\newcommand{\XPL}[4]{\langle #1, #2 \rangle_{\XSL{#3}{#4}}}




\newcommand{\XSP}[1]{X_{#1}^+}
\newcommand{\XNP}[2]{\|#1\|_{\XSP{#2}}}
\newcommand{\XSM}[1]{X_{#1}^-}
\newcommand{\XNM}[2]{\|#1\|_{\XSM{#2}}}


\newcommand{\XSoo}[1]{\mathring{X}_{#1}}
\newcommand{\XMoo}[2]{[#1]_{\XS{#2}}}
\newcommand{\XNoo}[2]{\|#1\|_{\XS{#2}}}

%% time-space

% X^k

\newcommand{\TXS}[1]{L^2(\XS{#1})}
\newcommand{\TXM}[2]{[#1]_{\TXS{#2}}}
\newcommand{\TXN}[2]{\|#1\|_{\TXS{#2}}}
\newcommand{\TXSL}[2]{L_t^2\XS{#1}({#2})}
\newcommand{\TXNL}[3]{\|#1\|_{\TXSL{#2}{#3}}}

\newcommand{\TXSK}[2]{X_{#1}(\XS{#2})}
\newcommand{\TXMK}[3]{[#1]_{\TXSK{#2}{#3}}}
\newcommand{\TXNK}[3]{\|#1\|_{\TXSK{#2}{#3}}}

\newcommand{\TXSS}[1]{L^2(\XSS{#1})}
\newcommand{\TXMS}[2]{[#1]_{\TXSS{#2}}}
\newcommand{\TXNS}[2]{\|#1\|_{\TXSS{#2}}}

% C^k

\newcommand{\CXS}[1]{C^0(\XS{#1})}
\newcommand{\CXM}[2]{[#1]_{\CXS{#2}}}
\newcommand{\CXN}[2]{\|#1\|_{\CXS{#2}}}
\newcommand{\CXSL}[2]{C_t^0\XS{#1}({#2})}
\newcommand{\CXNL}[3]{\|#1\|_{\CXSL{#2}{#3}}}

\newcommand{\CXSK}[2]{C^{#1}(\XS{#2})}
\newcommand{\CXMK}[3]{[#1]_{\CXSK{#2}{#3}}}
\newcommand{\CXNK}[3]{\|#1\|_{\CXSK{#2}{#3}}}

\newcommand{\CXSS}[1]{C^0(\XSS{#1})}
\newcommand{\CXMS}[2]{[#1]_{\CXSS{#2}}}
\newcommand{\CXNS}[2]{\|#1\|_{\CXSS{#2}}}

%% parabolic

\newcommand{\PXS}[1]{TX_{#1}}
\newcommand{\PXM}[2]{[#1]_{\dot \PXS{#2}}}
\newcommand{\PXN}[2]{\|#1\|_{\PXS{#2}}}

\newcommand{\PXSL}[2]{\PXS{#1}({#2})}
\newcommand{\PXML}[3]{[#1]_{\dot \PXSL{#2}{#3}}}
\newcommand{\PXNL}[3]{\|#1\|_{\PXSL{#2}{#3}}}


%% parabolic-from 0

\newcommand{\PXSN}[1]{\PXS{#1} \cap L^2(X_\eps^0)}
\newcommand{\PXMN}[2]{[#1]_{\dot \PXSN{#2}}}
\newcommand{\PXNN}[2]{\|#1\|_{\PXSN{#2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Y-norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\YS}[1]{Y_{#1}}
\newcommand{\YM}[2]{[#1]_{\YS{#2}}}
\newcommand{\YN}[2]{\|#1\|_{\YS{#2}}}
\newcommand{\YP}[3]{\langle #1, #2 \rangle_{\YS{#3}}}

\newcommand{\YSL}[2]{\YS{#1}({#2})}
\newcommand{\YML}[3]{[#1]_{\YSL{#2}{#3}}}
\newcommand{\YNL}[3]{\|#1\|_{\YSL{#2}{#3}}}
\newcommand{\YPL}[4]{\langle #1, #2 \rangle_{\YSL{#3}{#4}}}

\newcommand{\YSS}[1]{Y_{#1*}}
\newcommand{\YMS}[2]{[#1]_{\YSS{#2}}}
\newcommand{\YNS}[2]{\|#1\|_{\YSS{#2}}}
\newcommand{\YPS}[3]{\langle #1, #2 \rangle_{\YSS{#3}}}


\newcommand{\YSP}[1]{Y_{#1}^+}
\newcommand{\YNP}[2]{\|#1\|_{\YSP{#2}}}
\newcommand{\YSM}[1]{Y_{#1}^-}
\newcommand{\YNM}[2]{\|#1\|_{\YSM{#2}}}

% homoegenous bc

\newcommand{\YSoo}[1]{\mathring{Y}_{#1}}
\newcommand{\YMoo}[2]{[#1]_{\YS{#2}}}
\newcommand{\YNoo}[2]{\|#1\|_{\YS{#2}}}

\newcommand{\PYSL}[2]{TY_{#1}({#2})}
\newcommand{\PYML}[3]{[#1]_{\dot \PYSL{#2}{#3}}}
\newcommand{\PYNL}[3]{\|#1\|_{\PYSL{#2}{#3}}}

%% time-space

% Y^k

\newcommand{\TYS}[1]{L^2(\YS{#1})}
\newcommand{\TYM}[2]{[#1]_{\TYS{#2}}}
\newcommand{\TYN}[2]{\|#1\|_{\TYS{#2}}}

\newcommand{\TYSK}[2]{Y_{#1}(\YS{#2})}
\newcommand{\TYMK}[3]{[#1]_{\TYSK{#2}{#3}}}
\newcommand{\TYNK}[3]{\|#1\|_{\TYSK{#2}{#3}}}

\newcommand{\TYSS}[1]{L^2(\YSS{#1})}
\newcommand{\TYMS}[2]{[#1]_{\TYSS{#2}}}
\newcommand{\TYNS}[2]{\|#1\|_{\TYSS{#2}}}

% C^k

\newcommand{\CYS}[1]{C^0(\YS{#1})}
\newcommand{\CYM}[2]{[#1]_{\CYS{#2}}}
\newcommand{\CYN}[2]{\|#1\|_{\CYS{#2}}}

\newcommand{\CYSK}[2]{C^{#1}(\YS{#2})}
\newcommand{\CYMK}[3]{[#1]_{\CYSK{#2}{#3}}}
\newcommand{\CYNK}[3]{\|#1\|_{\CYSK{#2}{#3}}}

\newcommand{\CYSS}[1]{C^0(\YSS{#1})}
\newcommand{\CYMS}[2]{[#1]_{\CYSS{#2}}}
\newcommand{\CYNS}[2]{\|#1\|_{\CYSS{#2}}}

%% parabolic

\newcommand{\PYS}[1]{TY_{#1}}
\newcommand{\PYM}[2]{[#1]_{\dot \PYS{#2}}}
\newcommand{\PYN}[2]{\|#1\|_{\PYS{#2}}}


%% parabolic-from 0

\newcommand{\PYSN}[1]{\PYS{#1} \cap L^2(Y_\eps^0)}
\newcommand{\PYMN}[2]{[#1]_{\dot \PYSN{#2}}}
\newcommand{\PYNN}[2]{\|#1\|_{\PYSN{#2}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Z-norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\ZS}[1]{Z^{#1}}
\newcommand{\ZM}[2]{[#1]_{\ZS{#2}}}
\newcommand{\ZN}[2]{\|#1\|_{\ZS{#2}}}
\newcommand{\ZP}[3]{\langle #1, #2 \rangle_{\ZS{#3}}}

\newcommand{\ZSL}[2]{Z^{#1}({#2})}
\newcommand{\ZML}[3]{[#1]_{\ZS{#2}{#3}}}
\newcommand{\ZNL}[3]{\|#1\|_{\ZS{#2}{#3}}}
\newcommand{\ZPL}[4]{\langle #1, #2 \rangle_{\ZS{#3}{#4}}}



